pyTTN: An Open Source Toolbox for Open and Closed System Quantum Dynamics Simulations Using Tree Tensor Networks

We present the Python Tree Tensor Network package (pyTTN) for the evaluation of dynamical properties of closed and open quantum systems that makes use of Tree Tensor Network (TTN), or equivalently the multi-layer multiconfiguration time-dependent Hartree (ML-MCTDH), based representations of wavefunctions. This package includes several features allowing for easy setup of zero- and finite-temperature calculations for general Hamiltonians using single and multi-set TTN ans\"atze with an adaptive bond dimension through the use of subspace expansion techniques. All core features are implemented in C++ with Python bindings provided to simplify the use of this package. In addition to these core features, pyTTN provides several tools for setting up efficient simulation of open quantum system dynamics, including the use of the TTN ansatz to represent the auxiliary density operator space for the simulation of the Hierarchical Equation of Motion (HEOM) method and generalised pseudomode methods; furthermore we demonstrate that the two approaches are equivalent up to a non-unitary normal mode transformation acting on the pseudomode degrees of freedom. We present a set of applications of the package, starting with the widely used benchmark case of the photo-excitation dynamics of 24 mode pyrazine, following which we consider a more challenging model describing the exciton dynamics at the interface of a $n$-oligothiophene donor-C$_{60}$ fullerene acceptor system. Finally, we consider applications to open quantum systems, including the spin-boson model, a set of extended dissipative spin models, and an Anderson impurity model. By combining ease of use, an efficient implementation, as well as an extendable design allowing for the addition of future extensions, pyTTN can be integrated in a wide range of computational modelling software.

==> old_text.tex <==


\pagebreak
a
\pagebreak
\color{red}
\section{Illustrative Applications: Open Quantum System Dynamics}
\subsection{Spin-Boson Model}
\begin{figure*}[t]
\includegraphics[width=0.95\textwidth]{Figures/sbm_zero_temp_results.pdf} 
\caption{\label{fig:sbm_zero_temp} Top) The converged polarisation dynamics of the spin-boson model at $T=0$ with $\omega_c=5$ and varying values for the Kondo parameter $\alpha$, obtained using (from left to right) the star, chain, interaction picture chain, and HEOM based approaches.  For the unitary dynamics based methods converged results were obtained using a subspace expansion tolerance of $10^{-6}$, where as a subspace expansion of $10^{-8}$ was necessary for convergence of the HEOM dynamics.  Bottom) The maximum bond dimension used to satisfy this truncation tolerance bound.
The results presented here were generated using the scripts \protect\path{pyttn/examples/oqs/sbm.py} and \protect\path{pyttn/examples/oqs/sbm_heom.py}. \lc{TO Do: update figure and include }} 
\end{figure*}
We now consider the spin-boson model, a prototypical open quantum system model, in which a single two-level system (TLS) is linearly coupled to a harmonic bath.\citep{garg1985,Leggett1987,nitzan2006,Weiss2012} The spin-boson model Hamiltonian may be written in the form
\begin{equation}
\hat{{H}}_s=\varepsilon\hat{{\sigma}}_{z}+\Delta\hat{{\sigma}}_{x}+\hat{{\sigma}}_{z}\sum_{k=1}^Ng_{k}(\hat{{a}}_{k}^{\dagger}+\hat{{a}}_{k})+\sum_{k=1}^N\omega_{k}\hat{{a}}_{k}^{\dagger}\hat{{a}}, \label{eq:sbm_hamiltonian_2}
\end{equation}
 where $\hat{{a}}_{k}^{\dagger}$ and $\hat{{a}_{k}}$ are
the bosonic creation and annihilation operators associated with the
$k$th bath modet, and 
\begin{equation}
\hat{{\sigma}}_{x}=\left|0\right\rangle \left\langle 1\right|+\left|1\right\rangle \left\langle 0\right| \text{ and }
\hat{{\sigma}}_{z}=\left|0\right\rangle \left\langle 0\right|-\left|1\right\rangle \left\langle 1\right|
\end{equation}
are Pauli matrices. 


In all calculations performed for the spin-boson model, we have considered an ML-MCTDH ansatz in which the system degree of freedom is directly connected to the root node, and the bath degrees of freedom are treated as a balanced binary tree that is connected to the system through the root node.  

\subsubsection{Unitary Dynamics}
\lc{to do:  
\begin{itemize}
    
    \item Convergence with respect to fixed bond dimension $\alpha=0.7$
    \item Convergence with respect to 
\end{itemize}}
\subsubsection{Zero Temperature Dynamics}

We start by considering the zero temperature dynamics of the spin-boson, with parameters taken from Ref.~\onlinecite{Strathearn2018}, that is $\epsilon=0$, $\Delta=0.5$, $\omega_c=5$ and we consider ranges of $\alpha\in[0.1,1.5]$.  In order to accurately capture the bath correlation function up to times $t=30$, we discretise the bath using a maximum frequency cutoff of $\omega_{max}=7.5\omega_c$, and a total of $300$ bath modes obtained using the orthogonal polynomial discretisation.  The effect of modes with frequency $\omega_i > \omega_{max}$ are approximated by performing a polaron transformation for these modes, and tracing out these modes in the resultant Hamiltonian.  This gives rise to a renormalisation of the tunnelling matrix element of the form \lc{add renormalisation}. We consider the time evolution of the system $\hat{S}_z$ operator, starting from an initially uncorrelated configuration in which the system is found in the $\ket{\uparrow}$ state and the bath is initially in the vacuum state.  All results presented in this section were generated with the script \path{pyttn/examples/oqs/sbm.py}.



\lc{Replace this section and the results with plots of maximum bond dimension as a function of time}
%The dynamics of the polarisation obtained using the star Hamiltonian and using $\chi=16$, is presented in Fig.~\ref{fig:sbm_zero_temp}, where we observe excellent agreement with the results presented in Ref.~\onlinecite{Strathearn2018}, showing the expected transition from the coherent, underdamped oscillations for $\alpha < 0.5$ to the incoherent overdamped decay for $\alpha > 0.5$.  Finally, at large $\alpha > 1$ we observe the expected trend towards the localised regime.  As expected, we find that the dynamics obtained using the three Hamiltonian geometries, agrees (well within the accuracy of the graphs shown here), however, subtle differences are observed in the convergence of the dynamics.  This is illustrated in the bottom panels of Fig.~\ref{fig:sbm_zero_temp}, where we plot the relative difference in magnetisation dynamics, defined by 
%\begin{equation}
%    \Delta \langle \hat{S}_z(t) \rangle =  \frac{\langle \hat{S}_z(t) \rangle_{16} - \langle \hat{S}_z(t) \rangle _{8}}{\mathrm{max}(\langle \hat{S}_z(t) \rangle_{16}) - \mathrm{min}(\langle \hat{S}_z(t) \rangle_{16})},
%\end{equation}
%obtained with a bond dimension of $\chi=8$ and $\chi=16$ for the star (left), chain (middle), interaction picture chain (right) Hamiltonians.  The results obtained using the chain geometry shows the largest deviation between the two sets of results, indicating that larger bond dimensions are required to obtain converged results, %disc

%In contrast, the interaction picture form of the chain Hamiltonian exhibits only very minor deviation in results obtained with the two bond dimensions.  Additionally, we note that the hSOP representation of the interaction picture chain Hamiltonian only requires the evaluation of two terms at each node compared to three at each node in the star form, and four at each node for the chain form, and as such, we observe a reduced computational cost associated with each step. These results suggest that, at least in this case, the interaction picture chain Hamiltonian is favourable compared to the more standard star and chain forms, consistent with results observed for finite temperature Debye baths in Ref.~\onlinecite{ICCHAIN}.

%We note that here we have only considered the case of a balanced binary tree for representing the bath degrees of freedom, and that this conclusion may depend on the specific choice of the tensor network structure. In particular, the choice of an MPS with optimised boson basis may work better in capturing the correlation observed for the chain Hamiltonian with its linear coupling topology.  A careful, and more general, comparison of the convergence of the various approaches, and other potentially more advanced unitary bath transformations is beyond the scope of this manuscript and left as future work. 


\subsubsection{Finite Temperature Correlation Functions}
We next consider the application of this code to evaluate finite temperature correlation functions commonly explored within open quantum system calculations.  
All results presented in this section were generated with the scripts \path{pyttn/examples/oqs/sbm.py} and \path{pyttn/examples/oqs/sbm_heom.py}.

Here we consider two different approaches for evaluating such correlation functions, namely the use of the thermofield dynamics\cite{x} and a tensor network based solution of the hierarchical equations of motion approach\cite{x}.  In the thermofield dynamics approach, we consider a 

As in the zero temperature case, the thermofield Hamiltonian can freely be transformed to the chain geometry, as is employed in the T-TEDOPA method\cite{PhysRevLett.123.090402}, or the interaction picture of the chain geometry. 

Within the thermofield theory based approach, the coupling constants, the coupling constants associated with bosons with low onsite energy in the star representation become large due to the temperature dependent bose function contribution.  Accurate treatment of these requires the use of very large primitive basis sizes (that grow larger with increasing temperature).  In contrast, the chain and interaction picture chain geometries have been show to require 
\begin{figure}[h]
\includegraphics[width=0.95\columnwidth]{Figures/sbm_thermofield.pdf}
\caption{\label{fig:sbm_thermofield} Top) The polarisation dynamics of the spin-boson model obtained with thermofield theory and the interaction picture chain Hamiltonian with $\omega_c=5$ at varying values of $\beta$ and $\alpha$.  Bottom) Deviation between results obtained using a maximum bond dimension of $32$ and $16$ for $\beta=5$, $48$ and $32$ for $\beta=1$ and $64$ and $48$ for $\beta=0.2$ for the star (left), chain (centre), and interaction picture chain (right) forms of the Hamiltonian. The results presented in this figure were generated using the script \protect\path{pyttn/examples/oqs/sbm.py}.}
\end{figure}

\subsubsection{Non-Unitary Dynamics Methods}

\lc{Have decided to combine the approach Combine much of this discussion into the earlier section}
%\subsection{HEOM Dynamics}
%\begin{figure}[h]
%\includegraphics[width=0.95\columnwidth]{Figures/sbm_heom_zero_t_results.pdf} 
%\caption{\label{fig:sbm_heom_zero_temp} Top) Convergence of the dynamics of the zero temperature spin boson model considered in Fig.~\ref{fig:sbm_zero_temp} obtained using the Free-Pole HEOM methods as implemented within pyTTN, for varying subspace expansion tolerances. Bottom) The maximum bond dimension required for converged dynamics obtained with a subspace expansion tolerance of $10^{-6}$ and maximum allowed bond dimension of 100. 
%The results presented here were generated using the script \protect\path{pyttn/examples/oqs/sbm_heom.py}.}
%\end{figure}

%We now revisit the zero and finite temperature quench dynamics considered in the Sec.~\ref{}, using the HEOM method implemented within pyTTN.  In Fig.~\ref{fig:sbm_heom_zero_temp}, we present the convergence of the dynamics of the ohmic spin-boson model with an exponential cutoff with $\omega_c=5$, $\Delta=0.5$, and various values for the Kondo parameter, $\alpha$, as a function of the subspace expansion cutoff tolerance.  Here we observe that we are able to reproduce the zero temperature dynamics obtained using the unitary approaches (Fig.~\ref{fig:sbm_zero_temp}). However, it is worth noting that considerably smaller cutoff tolerances are required to produce accurate dynamics, with deviations being observed between results with tolerances of $10^{-7}$ and $10^{-8}$, compared to the unitary dynamics case.



%In these calculations we made use of the AAA algorithm to discretise the bath, with a cutoff tolerance of $10^{-5}$, leading to a total of 19 contributions to the sum-of-exponential decomposition of the bath correlation function, and consequently 38 total effective bosons to treat. This is a considerable reduction from the $300$ used in the unitary dynamics approaches above that were required to accurately capture the bath correlation function over the same time period.  This highlights the major advantage of HEOM based approaches for addressing open quantum system methods with continuous spectral densities, the ability to accurately reproduce continuous spectral densities with few modes.  We note that more compact representations valid over a specific time period can be obtain using other decomposition schemes such as the ESPRIT method, leading to potentially more efficient HEOM calculations. 

%In the bottom panel of  Fig.~\ref{fig:sbm_heom_zero_temp}, we present the maximum bond dimension used throughout the network when using a subspace expansion tolerance of $10^{-7}$ (bottom panel).  Here we find that the bond dimension requirements are considerably larger than was required for the zero temperature unitary dynamics case, leading to considerably higher costs in the updating of individual site tensors in the tree tensor network.  

%Need to discuss the finite temperature dynamics
%We next consider the dynamics 
%This story changes somewhat when we move to finite temperature dynamics.  In Fig.~\ref{fig:sbm_heom_finite_temp}, we present the dynamics of the ohmic spin-boson model with an exponential cutoff with $\omega_c=5$, $\Delta=1$, for various value of the Kondo parameter, $\alpha$, and at various temperatures.  Here we once again, observe excellent agrem

%dynamics obtained using the FP-HEOM method. We observe excellent agreement between the FP-HEOM and unitary dynamics methods implemented within pyTTN demonstrating its suitability for simulating both approaches to open quantum system dynamics.  
In these FP-HEOM calculation we have used a tolerance in the AAA algorithm of $10^{-5}$ leading to a total of 38, 32, 38, 36 (for $T=0$, $\beta=5, 1, 0.2$, respectively) effective bosonic modes in the HEOM representation.  This is considerably fewer than are required to obtain accurate dynamics using the unitary dynamics methods discussed above (requiring 300 to access the $T+0$ modes to accurately represent correlation functions, see Supplementary Information Sec.~\ref{}).  This highlights the main advantage of the FP-HEOM approach over the unitary dynamics approaches discussed above, namely the efficiency with which complex frequency bosons are able to represent decaying oscillations compared to stand 




%At zero temperature, we observe rather rapid growth in bond dimension with the HEOM approach, finding considerably larger bond dimension requirements to accurately capture the dynamics compared to the star and interaction picture chain representations.  At

%\begin{figure*}[t]
%\includegraphics[width=0.85\textwidth]{Figures/sbm_heom_finite_t_results.pdf} 
%\caption{\label{fig:sbm_heom_finite_temp} Top) Convergence of the dynamics of the spin boson model considered in Fig.~\ref{fig:sbm_thermofield} for varing $\beta=5$ (left), $\beta=1$ (centre), and $\beta=0.2$ (right), obtained using the Free-Pole HEOM methods as implemented within pyTTN, for varying subspace expansion tolerances. Bottom) The maximum bond dimension required for converged dynamics obtained with a subspace expansion tolerance of $10^{-6}$ and maximum allowed bond dimension of 100. 
%The results presented here were generated using the script \protect\path{pyttn/examples/oqs/sbm_heom.py}.}
%\end{figure*}


%However, for the cases considered here, we find similar order of magnitude runtime requirements due to the significant reduction in the number of bath modes required within the HEOM problem.  This highlights that while HEOM + tensor network approaches may provide significant reductions in the number of modes needed to treat an open quantum system, whether or not this leads to significant reductions in runtime depends strongly on the nature of the problem being considered. 


\color{black}
